High-precision Hardware Oscillators Ensemble for GNSS Attack Detection

A wide gamut of important applications rely on global navigation satellite systems (GNSS) for precise time and positioning. Attackers dictating the GNSS receiver position and time solution are a significant risk, especially due to the inherent vulnerability of GNSS systems. A first line of defense, for a large number of receivers, is to rely on additional information obtained through the rich connectivity of GNSS enabled platforms. Network time can be used for direct validation of the GNSS receiver time; but this depends on network availability. To allow attack detection even when there are prolonged network disconnections, we present a method based on on-board ensemble of reference clocks. This allows the receiver to detect sophisticated attacks affecting the GNSS time solution, independently of the specific attack methodology. Results obtained with Chip-Scale Oven Compensated Oscillators (CS-OCXO) are promising and demonstrate the potential of embedded ensembles of reference clocks, detecting attacks causing modifications of the receiver time offset as low as 0.3us, with half the detection latency compared to related literature.

==> attack_description.tex <==
The attacks tested against the defense method are based on the publicly available TEXBAT scenarios \cite{Humphreys2012}. Such scenarios involve static or mobile receivers, with attackers that focus on position or time tampering. Each attack scenarios is also complemented by a ground truth case of absence of adversary, which is used as a validation case. Figure \ref{fig:adversary-player} shows the test setup used to play the adversarial traces. While the TEXBAT scenarios cover a wide range of potential adversaries and mobility scenarios, they are both limited in duration and objective of the spoofer. The lack of flexibility in changing the spoofing parameters is a strong limitation in testing variations of the same attack. 



\begin{figure}
    \centering
  \includegraphics[width=0.7\linewidth]{figures/adversary-player.pdf}
  \caption{Setup used to evaluate different adversarial scenarios. The SDR timing is provided by a precision rubidium oscillator.}
  \label{fig:adversary-player}
\end{figure}
